State-of-the-art Speech Recognition With Sequence-to-Sequence Models

Attention-based encoder-decoder architectures such as Listen, Attend, and Spell (LAS), subsume the acoustic, pronunciation and language model components of a traditional automatic speech recognition (ASR) system into a single neural network. In previous work, we have shown that such architectures are comparable to state-of-theart ASR systems on dictation tasks, but it was not clear if such architectures would be practical for more challenging tasks such as voice search. In this work, we explore a variety of structural and optimization improvements to our LAS model which significantly improve performance. On the structural side, we show that word piece models can be used instead of graphemes. We also introduce a multi-head attention architecture, which offers improvements over the commonly-used single-head attention. On the optimization side, we explore synchronous training, scheduled sampling, label smoothing, and minimum word error rate optimization, which are all shown to improve accuracy. We present results with a unidirectional LSTM encoder for streaming recognition. On a 12, 500 hour voice search task, we find that the proposed changes improve the WER from 9.2% to 5.6%, while the best conventional system achieves 6.7%; on a dictation task our model achieves a WER of 4.1% compared to 5% for the conventional system.

==> related.tex <==
\section{Related Work\label{sec:related}}
%Budget: 0.5 page

There has been a variety of sequence-to-sequence models explored for speech, which differ in the interaction between the encoder and decoder. One of the early approaches introduced in the literature was Recurrent Neural Network Transducer (RNN-T) \cite{Graves12}, which has a separate encoder and decoder, which is combined by a linear prediction network. More recently, atttention-based models \cite{Jan15} where the encoder feeds the encoder have been explored, including Listen, Attend and Spell \cite{Chan15}, Neural Transducer \cite{Jaitly15}, Monotonic Alignments \cite{Colin17} and Recurrent Neural Aligner (RNA) \cite{Hasim17}. In addition, there have been a few papers comparing the performance different approaches for large scale speech tasks \cite{RohitSeq17,RohitAnal17,Battenberg17}. The main theme of these comparison papers indicates that attention-based models like LAS outperform separate encoder-decoder architectures like RNN-T, or architectures where attention is computed over a small window, such as RNA, Monotonic Aligment and NT. However, none of these papers is able to show that LAS can outperform a competitive state of the art LVCSR system. Building on the above work, we also explore LAS as the sequence-to-sequence model in this paper
\TS{fix slightly}

Initial work in sequence-to-sequence modeling  looked at seq2seq models with graphemic units, thus removing the need for a lexicon and languade model,
More recently,there has been work exploring different types of units for sequence-to-sequence models, including word piece models \cite{Yonghui16} and context-independent phones \TS{CITE TARA}. In \cite{Rao17}, the authors show that RNN-T trained with WPM can come very close to the performance of a state-of-the-art system. 

Error analysis of sequence-to-sequence models indicates that the models make many language modeling errors. This is likely because the model is trained on much less data compared to the LM, which can see trillions of text-only queries. To address these issue, there has been work exploring how to incorporate an external LM, including a log linear interpolation of the sequence-to-sequence model with an external LM during beam search \cite{Jan17}, Cold Fusion \cite{ColdFusion17}, Merl paper. While these papers have shown improvements by incorporating an external LM, again nobody has shown improvements compared to a competitive state of the art LVCSR system.

Our work differs from the above papers in that we break down and analyze diferent factors, i.e. training algorithm, unit inventory, language model integration, to obtaa model which improves over a strong baseline system. \TS{fix this to work more with intro and stress novelty}




%
%a lot of these paeprs look at small vocabulary tasks
%Cite seq2seq recent advances:
%\begin{itemize}
%\item Transformers
%\item Matt EMBR?
%\item Our interspeech papers
%\item Cold Fusion
%\item Our ICASSP co-submissions: LM, NT, Phones, Attention, MBR.
%\end{itemize}

